Synchronization and Localization in Ad-Hoc ICAS Networks Using a Two-Stage Kuramoto Method

To enable Integrated Communications and Sensing (ICAS) in a peer-to-peer vehicular network, precise synchronization in frequency and phase among the communicating entities is required. In addition, self-driving cars need accurate position estimates of the surrounding vehicles. In this work, we propose a joint, distributed synchronization and localization scheme for a network of communicating entities. Our proposed scheme is mostly signal-agnostic and therefore can be applied to a wide range of possible ICAS signals. We also mitigate the effect of finite sampling frequencies, which otherwise would degrade the synchronization and localization performance severely.

==> content/figures/simulation/finite_sampling_no_drift_compensation/content/pulse_durations_defs.tex <==
\newcommand{\PlotReferenceDurationValue}{150.10\xspace}

\newcommand{\PlotReferenceDurationUnit}{ns\xspace}



==> content/figures/simulation/finite_sampling_with_continous_drift_compensation/content/instantaneous_frequencies_defs.tex <==
\newcommand{\PlotReferenceFrequencyValue}{7224.767\xspace}

\newcommand{\PlotReferenceFrequencyUnit}{kHz\xspace}



==> content/figures/simulation/finite_sampling_with_continous_drift_compensation/content/pulse_durations_defs.tex <==
\newcommand{\PlotReferenceDurationValue}{138.41\xspace}

\newcommand{\PlotReferenceDurationUnit}{ns\xspace}



==> content/figures/simulation/finite_sampling_with_continous_drift_compensation/content/relative_position_errors_defs.tex <==
% empty


==> content/figures/simulation/finite_sampling_with_continous_drift_compensation/content/transmit_deviations_defs.tex <==
% empty


==> content/figures/simulation/infinite_sampling/content/instantaneous_frequencies_defs.tex <==
\newcommand{\PlotReferenceFrequencyValue}{7464.103\xspace}

\newcommand{\PlotReferenceFrequencyUnit}{kHz\xspace}



==> content/figures/simulation/infinite_sampling/content/pulse_durations_defs.tex <==
\newcommand{\PlotReferenceDurationValue}{133.97\xspace}

\newcommand{\PlotReferenceDurationUnit}{ns\xspace}



==> content/figures/simulation/infinite_sampling/content/relative_position_errors_defs.tex <==
% empty


==> content/figures/simulation/infinite_sampling/content/transmit_deviations_defs.tex <==
% empty


==> content/sim_parameters/common_config_table.tex <==
% This file is auto-generated by '..\..\..\simulation\impl\config_to_latex.py'
% Do not edit directly.

\begin{table}[H]
  \centering
  \begin{tabular}{ll}
    \toprule
    parameter&value\\ 
    \midrule
    Sampling frequency \SamplingFrequency{} & 800.00~MHz \\ 
    Sampling factor \SamplingFactor{} & 8 \\ 
    Number of hosts & 4 \\ 
    position of host 0 & \ensuremath{\left[0~\text{m}, 0~\text{m}, 0~\text{m}\right]\mTr} \\ 
    position of host 1 & \ensuremath{\left[30~\text{m}, 10~\text{m}, 0~\text{m}\right]\mTr} \\ 
    position of host 2 & \ensuremath{\left[10~\text{m}, -30~\text{m}, -10~\text{m}\right]\mTr} \\ 
    position of host 3 & \ensuremath{\left[20~\text{m}, -25~\text{m}, 20~\text{m}\right]\mTr} \\ 
    \bottomrule
  \end{tabular}
  \caption{Simulation parameters common to all hosts}\label{tab:commonsimparams}
\end{table}

